Exploring cosmic homogeneity with the BOSS DR12 galaxy sample

In this study, we probe the transition to cosmic homogeneity in the Large Scale Structure (LSS) of the Universe using the CMASS galaxy sample of BOSS spectroscopic survey which covers the largest effective volume to date, $3\ h^{-3}\ \mathrm{Gpc}^3$ at $0.43 \leq z \leq 0.7$. We study the scaled counts-in-spheres, $\mathcal{N}(<r)$, and the fractal correlation dimension, $\mathcal{D}_2(r)$, to assess the homogeneity scale of the universe using a $Landy\ \&\ Szalay$ inspired estimator. Defining the scale of transition to homogeneity as the scale at which $\mathcal{D}_2(r)$ reaches 3 within $1\%$, i.e. $\mathcal{D}_2(r)>2.97$ for $r>\mathcal{R}_H$, we find $\mathcal{R}_H = (63.3\pm0.7) \ h^{-1}\ \mathrm{Mpc}$, in agreement at the percentage level with the predictions of the $\Lambda$CDM model $\mathcal{R}_H=62.0\ h^{-1}\ \mathrm{Mpc}$. Thanks to the large cosmic depth of the survey, we investigate the redshift evolution of the transition to homogeneity scale and find agreement with the $\Lambda$CDM prediction. Finally, we find that $\mathcal{D}_2$ is compatible with $3$ at scales larger than $300\ h^{-1}\ $Mpc in all redshift bins. These results consolidate the Cosmological Principle and represent a precise consistency test of the $\Lambda CDM$ model.

==> Chapter_four.save.tex <==
\section{Theoretical Model}\label{sec:Theoretical Model}
\subsection{Prediction for $\xi(r),\mathcal{N}(<r),\mathcal{D}_2(r)$}
	
We use the CLASS software \cite{CLASS} to compute the $\Lambda$CDM theoretical prediction for the two-points correlation function and the observables we consider in the analysis. CLASS computes the theoretical matter power spectrum,  $P^{(r)}_{\delta\delta}(k)$, where the exponent $(r)$ indicates that it is calculated in {\em configuration space}, i.e.~without redshift space distortions. We expect our measurement to be sensitive to redshift space distortions (RSD) and we therefore model them in order to be able to predict the {\em redshift space} $P^{(s)}_{gg}(k)$ galaxy power spectrum (hence the $(s)$ exponent) and account for RSD in our data analysis. The redshift space distortions act on two different scales and we use a model for each of these scales:
\begin{itemize}
\item On large scales, galaxies are falling into large gravitational potentials, which tends to sharpen their distribution in the line of sight in redshift space. This is known as the Kaiser effect~\cite{Kaiser}, which results in:
	\begin{equation}\label{eq:largeRDS}
		P^{(s)}_{gg}(k,\mu;b) = b^{2}  (1+\beta \mu^{2})^{2} \ P^{(r)}_{\delta\delta}(k)
	\end{equation}
where $b$ is the linear (scale independent)  bias between galaxy and matter distributions, $\beta = f/b$ where $f$ is the growth rate,% growth factor is D <==
which can be approximated by $f \approx \Omega^{0.55}_{m}(z)$\cite{Growth} and $\mu=cos\theta$, $\theta$ being the angle from the line-of-sight.

\item On small scales, galaxies have a velocity dispersion whose projection on the line of sight in redshift space gives rise to the finger of god effect (FoG). These distortions can be modeled with a simple Gaussian orientation-dependent and scale-dependent damping model taking into account the pairwise peculiar velocity dispersion of the galaxies $\sigma_{p}$  \cite{FoG}:
	\begin{equation}\label{eq:Dumbing}
		D(k,\mu;\sigma_{p}) = e^{ - \frac{1}{2} \left( \frac{k\sigma_{p}\mu}{H_{0}} \right)^{2}}
	\end{equation}
This damping factor represents well actual data down to scales where $k\sigma_{p} \sim H_{0}$ \cite{FoG}.  % down to ?
\end{itemize}

Finally, accounting for both effects and integrating over all orientations w.r.t. the line of sight, the redshift-space galaxy power spectrum reads:
	\begin{equation} \label{eq:LSS_RSD}
		P^{(s)}_{gg}(k;b,\sigma_{p}) = b^{2} \int^{1}_{0} (1+\beta \mu^{2})^{2} D(k,\mu;\sigma_{p}) d\mu \ P^{(r)}_{\delta\delta}(k)
	\end{equation}
which can be integrated analytically over $\mu$ leading to:
\begin{eqnarray}
P^{(s)}_{gg}(k;b,\sigma_{p})=P^{(r)}_{\delta\delta}(k) \times \frac{b^2 H_0}{2k^5\sigma_p^5} \times  &\left[  -2\exp\left(-\frac{k^2 \sigma ^2}{2 H_0^2}\right) k \beta \sigma_p H_0 \left( k^2 (2+\beta) \sigma_p^2 + 3\beta H_0^2\right) \right. \nonumber \\
& \left. +\sqrt{2\pi} \mathrm{Erf}\left( \frac{k\sigma_p}{\sqrt{2}H_0}\right) \left(k^4 \sigma_p^4 + 2k^2\beta\sigma_p^2 H_0^2 + 3\beta^2 H_0^4\right)
\right] \label{eq:model}
\end{eqnarray}	
%
Applying a fast Fourier transform to equation (\ref{eq:model}) result in the two-point correlation function with two parameters $[b, \sigma_p]$:
	\begin{equation}\label{eq:fit-model}
		\xi^{(s)}(r;b,\sigma_{p}) = FFT\left[ P_{gg}^{(s)}(k;b,\sigma_{p})\right]
	\end{equation}
Then we use equation (\ref{eq:Counts}) and (\ref{eq:Fractal}) to compute the $\Lambda$CDM prediction for $\mathcal{N}(<r)$ and $\mathcal{D}_{2}(r)$.

\iffalse
One may, however, question the strict necessity of including these redshift space distortion corrections in our large scale homogeneity analysis. In order to address this question, we have made a simple test: we calculate the ratio between the theoretical homogeneity scale (as defined in Eq.~\ref{eq:RH-definition}) with or without accounting for redshift space distortions. We use a range of values for the RSD parameters around the typical $(b\approx 1.95,  \sigma_{p} \approx 300\ h\ km/s)$, \cite{Sigma}. This percentage ratio is shown in Fig.~\ref{fig:Theory-Correction} for our second redshift bin (for which the effect is expected to be the largest) and turns out to be ranging between 15 and 25\% depending on the value of the galaxy bias. We observe no significant effect on the ratio regarding the galaxy velocity dispersion. \textbf{Although, we need to take it into account because it is degenerated with bias parameter}. The redshift space distortion effects are therefore not negligible when comparing the homogeneity scale for data and $\Lambda$CDM predictions, which justifies the use of this model for our analysis. 
	\begin{figure}[h!]
	\centering
	\includegraphics[width=100mm]{images/Model-correction}
	\caption{Test of necessity of RSD modelling: We show the percentage ratio of the homogeneity scale defined in Eq.~\ref{eq:RH-definition} without and with redshift space distortions accounted for according to Eq.\ref{eq:model}. The effect ranges from 15 to 25\% and varies according to the bias parameter and is therefore not negligible. \label{fig:Theory-Correction}}
		\end{figure}
\fi

\subsection{Estimator-Reconstruction}
	{\color{blue} 
The estimators presented in section \ref{subsect:Estimators} measure the clustering properties of the galaxy distribution, we need to convert them into estimators that describe the clustering properties of the total matter distribution. We fit the redshift distortion parameters ($\textbf{p}_{rsd} = [b,\sigma_p]$) to $\xi(r)$ in the range $1 \ h^{-1} Mpc\ <r<40 \ h^{-1} Mpc $ .


Thus, we perform the following procedure for the reconstructions of the estimators to those for the total matter distribution. We estimate the redshift distortion parameters ($\textbf{p}_{rsd} = [b,\sigma_p]$) where $b$ is  the galaxy bias and $\sigma_{p}$ peculiar velocities . Having the RSD parameters we model our Matter distribution estimator in the following manner:
	\begin{equation}\label{eq:convMatter}
		\hat{\mathcal{N}}(<r) =\frac{ \mathcal{N}^{Linear}_{\delta\delta}(<r;b=1,\sigma_p=0) -1 }{ \mathcal{N}^{RSD}_{gal}(<r;b,\sigma_{p}) -1 } * \left[ \hat{\mathcal{N}_{gal}}(<r) - 1 \right]+ 1
	\end{equation} 
	\paragraph{} Where $\mathcal{N}^{Linear}_{\delta\delta}(<r;b=1,\sigma_p=0)$ is the prediction for the \textit{scaled count-in-sphere} for the total matter distribution in Linear Theory without Redshift Space distortions while  $\mathcal{N}^{RSD}_{gal}(<r;b,\sigma_{p})$ is the prediction for the \textit{scaled count-in-sphere} for the galaxy distribution accounting for redshift space distortions. Then the reconstructed \textit{fractal correlation dimension} $\mathcal{D}_{2}(r)$ follows from equation \ref{eq:Fractal}.
	}


==> Chapter_two.save.tex <==
\section{Dataset}
	\subsection{The BOSS survey}
	\paragraph{}The Baryon Oscillation Spectroscopic Survey (BOSS) is dedicated to study the 3D distribution of $\sim1.4\times10^{6}$ galaxies and $\sim10^{5}$ quasars and their Lyman-a forests within an effective area of $\sim10000 deg^{2}$ \cite{BOSS-DR12}.  In the focal plain of the telescope 1000 optical fibers are positioned on drilled aluminium plates allowing to gather 1000 spectra per exposure~\cite{spectra} achieving a typical redshift uncertainty of a few tens on $\mathrm{km.s^{-1}}$~\cite{reso_z}. Using imaging data from SDSS-I-II and SDSS-III/BOSS in u,g,r,i,z~\cite{imaging}, massive galaxy targets are selected~\cite{Target-Selection} through several colour cuts designed to keep targets in redshifts between $0.43<z<0.7$ and keeping a constant stellar mass limit according to a passively evolving model \cite{Maraston}. The large masses ensure a strong bias with respect to the underlying Dark Matter field, allowing a high signal to noise ratio on the two-point correlation function. The resulting sample of galaxies is called CMASS and consists in $~\sim 10^6$ galaxies with accurate spectroscopic redshifts. The CMASS sample has been used to measure the Baryonic Acoustic Oscillation feature (BAO) with unprecedented accuracy allowing to put strong constraints on the cosmological parameters~\cite{BAOcosmo}. We use the same galaxy sample to perform our measurement of the transition to homogeneity.% Is the large mass ~ strong bias ~ high signal to noise ratio of BAO, affect our analysis?
	
We use the catalogue of weights according to BOSS-collaboration ~\cite{Target-Selection} given by the equation:
	\begin{equation}\label{eq:weights}
		w_{gal} = (w_{cp} + w_{noz} - 1)*w_{star}*w_{see}*w_{fkp}
	\end{equation}
These weights are important for several reasons. The $w_{cp}$ accounts for the fact that one cannot assign optical fibers to two targets that are closer than $62''$ due to plate and optical fiber constrains. The  $w_{noz}$ accounts for redshift failure of the targets. Finally, $w_{star}$ and $w_{see}$ account for correcting the observed correlation between the observed galaxy number density  and the stellar density and seeing that both reduce the area on the sky available for detecting galaxy targets. Moreover, in order to guarantee minimum variance on the two-point correlation function estimator, we use the FKP weighting scheme $w_{fkp}$~\cite{FKP}.

	\begin{table}[h!]
		\begin{center} 
		\begin{tabular}{ *3c } 
	 	$z$   & NGC & SGC  \\ 
	 	\hline 
		0.430-0.484 & 101,383  & 40,170   \\ 
	 	0.484-0.538 & 174,468  & 63,518   \\ 
	 	0.538-0.592 & 151,084  & 56,805   \\ 
		0.592-0.646 & 97,155    & 37,179   \\ 
		0.646-0.700 & 47,289    & 17,899   \\ 
		0.430-0.700 & 571,379  & 215,571 \\ 
	 	\hline
		\end{tabular}
		\end{center} 
	\caption{\label{tab:zbins} DR12 data sample divided on 5 redshift bins on North and South Galactic Caps.}
	\end{table}	
	
	\subsection{Homogeneity study data sample}
	\paragraph{}We divide our data sample into 5 redshift regions as shown in table \ref{tab:zbins} to study the evolution of the clustering of our galaxy sample. The CMASS galaxy sample is shown in figure \ref{fig:DR12} for the north and south galactic cap. We use the prediction of flat $\Lambda CDM$-model to convert the redshift measurements to comoving distances:
	\begin{equation}\label{eq:FRW}
		d_{comov} (z) =\frac{c}{H_{0}} \int_{0}^{z} \frac{dz'}{E(z')}
	\end{equation}
	where $E(z) = \sqrt{\Omega_{m,0}(1+z)^{3} + \Omega_{\Lambda} }$ and $H_{0} = 100h\ \mathrm{km/s/Mpc}$. The cosmological parameters used for calculating distances are given by equation (\ref{fid-cosmo}) and therefore assumes flatness.
	A final sample of total size of $5.1 h^{-3}Gpc^{3}$ \cite{Target-Selection} is obtained which is significantly larger than those used in previous studies such as $1 h^{-3}Gpc^{3}$ in WiggleZ or $0.6 h^{-3}Gpc^{3}$ of a BOSS LRG analysis \cite{Hogg} or the SDSS II with $0.25 h^{-3}Gpc^{3}$ \cite{Labini2}.


 

%	\begin{table}[t!] % Wrong Calculation of Volume: Overestimation! Due to the fact that the geometry is a cell
%		\begin{center} 
%		\begin{tabular}{ *7c } 
% 		\hline
%		XGC & \multicolumn{3}{c}{NGC} & \multicolumn{3}{c}{SGC}\\
%		\hline
	 	%$z$   & Number & $V [\mathrm{Gpc^3}]$ & $d_{eff} [\mathrm{Gpc^{-3}}]$ & Number & $V [\mathrm{Gpc^{3}}]$ & $d_{eff} [\mathrm{Gpc^{-3}}]$ \\ 
%	 	\hline 
%		0.430-0.484 & 101,383 & 1.09  &0.09  & 40,170  & 0.27 & 0.16 \\ 
%	 	0.484-0.538 & 174,468 & 1.44  &0.12  & 63,518  & 0.35 & 0.19 \\ 
%	 	0.538-0.592 & 151,084 & 1.83  &0.08  & 56,805  & 0.43 & 0.14 \\ 
%		0.592-0.646 & 97,155   &  2.27 &0.04  & 37,179  & 0.53 & 0.07 \\ 
%		0.646-0.700 & 47,289   &  2.75 &0.02  & 17,899  & 0.63 & 0.03 \\ 
%		0.430-0.700 & 571,379 &  9.28 &0.06  & 215,571& 2.14 & 0.10 \\ 
%	 	\hline
%		\end{tabular}
%		\end{center} 
	%\caption{\label{tab:zbins} DR12 data sample, their occupied volume and effective density on different redshift on North(NGC) and South(SGC) galactic caps.}
%	\end{table}	 
	

	\begin{figure}[ht!]
	\centering
	%\includegraphics[width=100mm]{images/dataDR12.png}
	\includegraphics[width=.49\linewidth, keepaspectratio]{images/dataDR12.png}
	\includegraphics[width=.49\linewidth, keepaspectratio]{images/dataDR12_histZ.pdf}	
	\caption{\label{fig:DR12} Right ascension and declination profiles (Left) , redshift distribution (Right) of the DR12 sample for the North (red) and South (blue) Galactic Caps. The dashed lines define the selected redshift region that we use in our analysis.}
	\end{figure}

%	\begin{figure}[h!]
%	\centering
%	\includegraphics[width=100mm]{images/dataDR12_histZ.pdf}
%	%\includegraphics[width=.49\linewidth, keepaspectratio]{images/dataDR12_histZ.png}
%	%\includegraphics[width=.49\linewidth, keepaspectratio]{images/dataDR12_histZ.png}
%	\caption{\label{fig:DR12} Redshift distribution of DR12 sample for both North (red) and South (blue) galactic caps. The dashed lines define the selected redshift region that we use in our analysis.}
%	\end{figure}

	\subsection{Mock-Catalogues}
	\paragraph{}Mock catalogues are an important tool for determining uncertainties in galaxy surveys and tuning data analysis pipelines. In our analysis we use 1000 Mock-Catalogues constructed with a quick-particle mesh algorithm ~\cite{QPM} for BOSS. These are expected to be more realistic than second-order Lagrangian perturbation theory based mocks, although not as accurate as the highly time consuming N-body based simulations. These catalogues use a different cosmology than the one we use in our analysis, but this is accounted for in our analysis:
	\begin{equation}\label{eq:qpmcosmo}
		(\Omega_{cdm},\Omega_{b},h,n_{s},\sigma_{8}) = (0.274,0.046,0.7,0.95,0.8)
	\end{equation}
	where $\sigma_{8}$ is the variance of the matter power spectrum computed in spheres of $8h^{-1}Mpc$.



==> bid <==
\section{Results}{\vspace{0.1pt}}

In this section, we present the results of our analysis. We determine the range in comoving distance for which we can measure $\mathcal N(<r)$ with our sample. We quantify the uncertainties in our measurements using mock catalogues. We then describe the observable reconstruction by using a Redshift Space Distortion(RSD) analysis. The estimation of the latter is crucial in order to convert our measurement of the galaxy tracer to a dark matter tracer of homogeneity. Finally, we compare our measurements of the dark matter homogeneity observables with the  $\Lambda$CDM predictions.

%--------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Analysis range}

Figure~\ref{fig:large_RR} shows the number density of random pairs, $dN/dr$, divided by $r^{2}$ and normalized such that at small scales it is unity. This scaled density is constant at small scales and then decreases with $r$ due to the finite size of the survey. We analyse  data up to a maximum $r=1300 h^{-1}$ Mpc, where the scaled density goes down to $1\%$. 
	
	\begin{figure}[h!]
	\centering
	\includegraphics[width=100mm]{images/largeRR.pdf}
	\caption{\label{fig:large_RR} Scaled number density of random pairs $r^{-2}dN/dr$ versus the comoving radius of spheres $r$, normalized to be unity at small $r$. }
	\end{figure}

%--------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Covariance matrices}\label{subsec:CovMat}

We use as set of 1000 QPM mock catalogues to estimate the covariance matrices. We compute our observables for each of the catalogues and derive the bin-to-bin covariance matrices for each of the relevant observables $\xi(r)$, $\mathcal{N}(<r)$ and $\mathcal{D}_{2}(r)$ 
using the various estimators % really ?  <==
that we introduced in section~\ref{sect:methodology}. 

%%%% COMMENT JC {\color{red} Here we need to discuss, I don't think I agree with what you do... On the data, we fit the bias and sigmap and then fit the theoretical model using the covariance matrix. So the covariance should be calculated on the mock doing the same: calculating the bias and sigmap on each mock. It seems that this is not what you are doing...}.

Fig.~\ref{fig:CorrMat} displays the resulting correlation matrices~\footnote{We show the correlation matrices, $\rho_{ij} = \frac{C_{ij}}{\sqrt{C_{ii}*C_{jj}}}$, rather than the covariance matrices since they have less dynamics.}
in the redshift bin $0.538 \le z \le 0.592$. The correlations matrices are similar in the other redshift bins.

	\begin{figure}[h]
	\centering
	\includegraphics[width=.32\linewidth, keepaspectratio]{images/corrmat_xi_ngc_z2_ls_without_rsd_pars.pdf}
	\includegraphics[width=.32\linewidth, keepaspectratio]{images/corrmat_nr_ngc_z2_JC_with_rsd_pars.pdf}
	\includegraphics[width=.32\linewidth, keepaspectratio]{images/corrmat_d2_ngc_z2_JC_with_rsd_pars.pdf}
	\caption{\label{fig:CorrMat} Correlation matrices for $\xi(r)$, $\mathcal{N}(<r)$ and $\mathcal{D}_{2}(r)$ for the total matter distribution in the redshift range $0.538 \le z \le 0.592$ .}
	\end{figure}
	
	\paragraph{} The correlations on $\mathcal{D}_{2}(r)$ observable are less than those of $\mathcal{N}(r)$.This is an expected effect since {\color{blue} $\mathcal{N}(r)$ is an integral of the $\xi(r)$ and adds up the correlation between the bins. Then, we differentiate $\mathcal{N}(r)$ to obtain $\mathcal{D}_2(r)$, which gives less correlations}. Regarding this result, we choose the $\mathcal{D}_{2}(r)$ observable to show the evolution of the homogeneity scale $R_{H}$ with redshift $z$ in section (\ref{subsec:RH}).


%--------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Homogeneity scale for galaxy distribution}\label{subsec:RH-gal}

We first compute  $\mathcal{N}^{gal}(<r)$  and $\mathcal{D}^{gal}_{2}(r)$ for the CMASS galaxy distribution using equation \ref{eq:Counts} and \ref{eq:Fractal}, without correcting for bias and redshift space distortions. This provides a measurement that does not rely on $\Lambda$CDM model to determine the bias. 
Results are shown in figure \ref{fig:RH-measure-GAL} for the $0.430 \le z \le 0.484$ redshift interval in the NGC.
The error bars were obtained from $1000$ QPM mock catalogues.

\begin{figure}[h!]
	\centering
	\includegraphics[width=.49\linewidth, keepaspectratio]{images/1_1_nrz0JC_ngc_GAL_90_600.pdf}
	\includegraphics[width=.49\linewidth, keepaspectratio]{images/1_1_d2z0JC_ngc_GAL_90_600.pdf}
	
	\caption{
\label{fig:RH-measure-GAL} Scaled counts-in-spheres, $\mathcal{N}(<r)$, (left) and fractal correlation dimension, $\mathcal{D}_{2}(r)$, (right). The black points with error bars are the result for the galaxy distribution in the NGC in the $0.430 \le z \le 0.484$ redshift bin. 
The blues lines are the best spline fit of the data.
The green lines are the results for the 1000 QPM mock catalogues. 
The red continuous line is the $\Lambda$CDM prediction for $b=1.95$ and $\sigma_p=379\  h$  km/s.
}
\end{figure}

The horizontal black-dashed lines in figure \ref{fig:RH-measure-GAL} indicate the value of the observable for an homogeneous distribution. The two observables reach homogeneity on large scales. 
The intersection of the data with the red-dashed lines  (at $\mathcal N=1.01$ and $\mathcal D_2=2.97$) defines the homogeneity scale. In order to determine it, we fit 14 data point around the intersection with a spline fit. The number of nodes of the spline fit is set to 5 in order to get an average $\chi^2$ equal to the number of degrees of freedom for the 1000 QPM mocks. The error on $R_{H}$ was obtained from the errors in the spline factors by error propagation.
For $\mathcal N$ we get $\mathcal{R}^{\mathcal{N}=1.01}_{H,gal}=136.5\pm6.7\ h^{-1}$ Mpc with a relative precision of $4.9\%$ . This is consistent with our $\Lambda$CDM model prediction $\mathcal{R}^{\mathcal{N}=1.01}_{H,gal}=xx$. For $D_2$ we get $\mathcal{R}^{\mathcal{D}_2=2.97}_{H,gal}=123.8\pm8.2\ h^{-1}$ Mpc with a relative precision of $6.4\%$ and also consistent with the prediction $\mathcal{R}^{\mathcal{D}_2=2.97}_{H,gal}=xx$.
We finally stress the fact that $1000$ QPM mock catalogues behave the same way as the data. 
	
{\color{red} 
Following the procedure in \citet{Laurent}, we can prove that the CMASS galaxy bias must be larger than unity by comparing the clustering measured by weak lensing \cite{BACON} to the galaxy clustering, measured on the CMASS sample.
Comparing the clustering of different tracers with different biases shows that the bias ratio is independent with scale. 
 Then one may assume that the bias measured at scales smaller than typically $40 h^{-1}Mpc$ can be used to correct for $\mathcal{N}(<r)$ and $\mathcal{D}_2$ on large scales.}


%--------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Determining redshift-space-distortion parameters}\label{subsec:RSD}
	
As illustrated in figure \ref{fig:bias}, we fit our model (Eq.~\ref{eq:fit-model}) % described in section \ref{sec:Theoretical Model} 
to the measured correlation function for the CMASS galaxy sample in order to determine the galaxy bias and velocity dispersion. As explained in Appendix \ref{APP:RSD-robust} we account for theoretical uncertainties on the RSD modeling by boosting the covariance matrix on the relevant small scales. We thus achieve a good $\chi^2/$n.d.f. in the range $[1,40]\ h^{-1}$ Mpc. 
This change in the covariance matrix has no 
The measurement of the homogeneity scale and each evolution remain independent of this change at the small scales of the covariance matrix.	


Results are given in table \ref{tab:bias}. The mean precision  is 2.6\% (NGC) and 4.1\% (SGC) for the bias and 12\% (NGC) and 23\% (SGC) for the velocity dispersion. 
The bias is in agreement with values obtained by several authors \cite{FoG,bias2010,bias2012,bias_stochastic} 
and the pairwise velocities is consistent with the typical CMASS galaxy sample  pairwise velocities $\sigma_{p} \approx 350\pm50\ h\ km/s$ \cite{Sigma}.  

		\begin{table}[h!]
	\setlength{\abovecaptionskip}{-8pt}
		\begin{center} 
		\begin{tabular}{*7c} 
		\hline
		%\toprule
		 & \multicolumn{3}{c}{NGC} & \multicolumn{3}{c}{SGC}\\
 		\hline
		%\midrule
%	 	z                   & b & $\sigma_{p} [h\ km/s]$ & $\chi_{red}^{2}$ & b & $\sigma_{p} [h\ km/s]$  & $\chi_{red}^{2}$ \\ 
%	 	\hline 
%		0.430-0.484 & $1.788 \pm 0.023$ & $348.3 \pm 13.6$   & 0.41 &\ \ $1.779 \pm 0.034$ & $341.3 \pm 21.1$   & 0.88 \\ 
%	 	0.484-0.538 & $1.738 \pm 0.021$ & $350.9 \pm 10.3$   & 0.57 &\ \ $1.733 \pm 0.032$ & $334.4 \pm 16.8$   & 0.65 \\ 
%	 	0.538-0.592 & $1.819 \pm 0.021$ & $356.8 \pm 12.2$   & 0.84 &\ \ $1.819 \pm 0.032$ & $334.9 \pm 18.8$   & 0.56 \\ 
%		0.592-0.646 & $1.854 \pm 0.022$ & $332.5 \pm 14.9$   & 1.37 &\ \ $1.860 \pm 0.035$ & $338.6 \pm 27.0$   & 0.78 \\ 
%		0.646-0.700 & $1.995 \pm 0.028$ & $334.2 \pm 29.5$   & 0.79 &\ \ $1.921 \pm 0.044$ & $299.1 \pm 54.4$   & 0.54 \\ 
	 	z                   & b & $\sigma_{p} [h\ km/s]$ & $\chi_{red}^{2}$ & b & $\sigma_{p} [h\ km/s]$  & $\chi_{red}^{2}$ \\ 
	 	\hline 
		0.430-0.484 & $1.879 \pm 0.023$ & $361.3 \pm 14.5$   & 0.44 &\ \ $1.872 \pm 0.035$ & $354.9 \pm 22.6$   & 0.85 \\ 
	 	0.484-0.538 & $1.846 \pm 0.021$ & $367.3 \pm 11.0$   & 0.67 &\ \ $1.840 \pm 0.032$ & $348.8 \pm 17.9$   & 0.66 \\ 
	 	0.538-0.592 & $1.944 \pm 0.021$ & $374.8 \pm 13.2$   & 0.91 &\ \ $1.943 \pm 0.032$ & $351.2 \pm 20.3$   & 0.59 \\ 
		0.592-0.646 & $1.995 \pm 0.022$ & $348.2 \pm 16.2$   & 1.47 &\ \ $2.001 \pm 0.035$ & $353.7 \pm 29.1$   & 0.79 \\ 
		0.646-0.700 & $2.153 \pm 0.028$ & $349.8 \pm 32.2$   & 0.79 &\ \ $2.081 \pm 0.045$ & $312.6 \pm 59.6$   & 0.50 \\ 
	 	\hline
		%\bottomrule
		\end{tabular}
		\end{center}
	\caption{\label{tab:bias} Fitted values of bias $b$ and velocity dispersion $\sigma_p$  in the different redshift bins, together with the corresponding reduced $\chi^{2}$ for $24$ degrees of freedom.}
	\end{table}	


\begin{comment} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[ht!]
	\setlength{\abovecaptionskip}{-100pt}
	\setlength{\belowcaptionskip}{10pt}
	\centering
	\vspace{-25mm}
	\includegraphics[width=100mm]{images/bias-fit.pdf}
\caption{\label{fig:bias} 
The correlation function of the CMASS galaxies in the $[0.538-0.592]$ redshift range. Data points have both their original error bars and the error bars enlarged to take into account the uncertainty of the RSD model on small scales (see appendix ). 
%The red line is the result of the fit performed over the range 
% $[1,40]\ h^{-1}$ Mpc (up to the vertical black-dashed line).
} 
\end{figure} 

%(see appendix~\ref{bla}).
%The red line is the result of the fit performed over the range 
%$[1,40]\ h^{-1}$ Mpc (up to the vertical black-dashed line).

%2*3.14/(240/(100*0.67) )/0.7 = 2.5 Mpc/h
	
%\end{document}

%--------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Homogeneity Scale Measurement on the Matter Distribution}	\label{subsec:RH}

We use equation (\ref{eq:convMatter}) with parameter $b$ and $\sigma_p$ obtained in section \ref{subsec:RSD} to transform $\mathcal{N}^{gal}(<r)$ into $\mathcal{N}(<r)$ for matter. We then use Eq 3.3 ~\ref{} to get $\mathcal{D}_{2}(r)$ for matter distribution. The result is shown in figure \ref{fig:RH-measure}.
	
\begin{figure}[h!]
	\centering
	\includegraphics[width=.48\linewidth, keepaspectratio]{images/DM_RH_mesure_nr_z2.pdf}
	%d2/nr _JC_Result_North_ 5/4 _multi_xibias_minuit_eff_0.0_1.0-40.0z_0.538_0.592
	\includegraphics[width=.48\linewidth, keepaspectratio]{images/DM_RH_mesure_d2_z2.pdf}
\caption{\label{fig:RH-measure} 
same as figure~\ref{fig:RH-measure-GAL} for matter distribution in the redshift interval $0.538 \le z \le 0.592$.
%The scaled counts-in-spheres $\mathcal{N}(<r)$ (left) and the {fractal correlation dimension} $\mathcal{D}_{2}(r)$ (right) for  matter distribution  (black error bars) im the $0.538 \le z \le 0.592$ on the NGC. }
%The matter distribution becomes homogeneous with increasing scales. See text for details.}
\end{figure}

{\color{blue} In order to perform the measurement of the Homogeneity scale, we fit a spline} 
\footnote{In order to be model independent}
{\color{blue} at each observable around the nominal values of homogeneity according to equation ($\ref{eq:RH-definition}$), resulting in 6 data points.} 

	We take care of the fact that we perform the fit on scales  $r=[40,100]h^{-1}Mpc$ in order to be independent from the scales of the measurement of the $\textbf{p}_{rsd}$-parameters (scales $r<40\ h^{-1}Mpc$). The number of nodes of the spline are tuned on the $1000$ QPM mock catalogues. The fits performed with the covariance matrices whose correlations matrices are described in section $\ref{subsec:CovMat}$. The error bars on $R_{H}$ where calculated from the error bars from the spline-factors with error propagation. 

	{\color{red} We observe the same results for the observables of the Homogeneity Scale for the matter distribution as the one obtained for the galaxy distribution as explained in section \ref{subsec:RH-gal}. The homogeneity of the matter distributions is reached in asymptotically on large scales. This shows that the inhomogeneity of the structures of matter on small scales vanishes on larges scale.}
	
																		                                   %(61.9-61.6)/61.6			0.8/61.9												%(67.4-67.0)/67.0 1.6/67.4
	%We measure, for the matter distribution, $\mathcal{R}^{\mathcal{D}_2=2.97}_{H}=61.8\pm0.8\ h^{-1}Mpc$ at an accuracy $0.5\%$ and precision $1.3\%$, while  $\mathcal{R}^{\mathcal{N}=1.01}_{H}=66.7\pm1.6\ h^{-1}Mpc$ at an accuracy $0.6\%$  and precision $2.4\%$, at the North Galactic Cap at redshift $0.538\le z < 0.592$.

	{\color{red} We measure, for the matter distribution, $\mathcal{R}^{\mathcal{D}_2=2.97}_{H}=63.9\pm0.6\ h^{-1}Mpc$ with precision $0.9\%$ with relative precision from the theoretical value $1.6\%$, while  $\mathcal{R}^{\mathcal{N}=1.01}_{H}=68.1\pm1.1\ h^{-1}Mpc$ with  and precision $1.6\%$ and a relative error from the theoretical value $6.6\%$, at the North Galactic Cap at redshift $0.538\le z < 0.592$ for the North and South Galactic Caps.}

	In order to describe the evolution of the homogeneity scale with redshift, we perform the homogeneity scale at $1\%$ measurement as defined by equation \ref{eq:RH-definition} in all redshift bins.	
	
	\begin{figure}[h!]
	\centering
	\includegraphics[width=100mm]{images/RH_vs_z_10.pdf}
	\caption{\label{fig:RH-z}The evolution of homogeneity scale with redshift $R^{\mathcal{D}_2=2.97}_{H}(z)$ as measured for $\mathcal{D}_{2}(r)$ at $1\%$. Green line correspond to the prediction of the $\Lambda CDM$-model. With error bars we denote the $DR12$ data. The shaded areas correspond to $1\sigma$ calculated from $1000$ QPM mock catalogues. The Homogeneity Scale is increasing with time. } % 0.84,0.57
	\end{figure}
	 
	 In figure \ref{fig:RH-z}, we show with blue the SGC, with red the NGC at $0.43\le z \le0.7$ and with purple the QSO measurement obtained by P. Laurent et Al. \cite{Laurent} at the north galactic cap at redshift $2.2\le z \le 2.8$. 
	 
	 We find that the measurement of the homogeneity scale as defined for $1\%$ via equation \ref{eq:RH-definition} is in excellent agreement with
%less than ($2\sigma$) away from
$\Lambda CDM$ prediction. For data measurements, we use the bias and peculiar velocities given in table \ref{tab:bias}. The homogeneity scale $R_{H}$ follows the $\Lambda CDM$-prediction with $\chi_{red}^{2} = 4.9/5$ for NGC and $\chi_{red}^{2} = 3.25/5$ for SGC. {\color{blue} By adding the observation from P.Laurent et al. we find $\chi_{red}^{2} =5.34/6$ for the NGC $\chi_{red}^{2} = 3.66/6$ for the SGC.}

	\begin{figure}[h!]
	\centering
	\includegraphics[width=100mm]{images/RH_vs_z_QSO_eff10.pdf}
	\caption{\label{fig:RH-z-QSO}Same as figure \ref{fig:RH-z} but adding the P.Laurent et al. observation at larger redshifts.}	
	\end{figure}
	
	 {\color{red} We also observe that the homogeneity scale $R_{H}$ is increasing with time as one expected from the $\Lambda CDM$ model prediction, as structures are growing with time. } 	

{\color{red} We summarise our results in table \ref{tab:RH-z} }

{\small
	\begin{table}[h!]
		\begin{center} 
		\begin{tabular}{*5c} 
		\hline
%		estim & \multicolumn{2}{c}{\textit{str}} & \multicolumn{2}{c}{\textit{cor}}\\
% 		\hline
%		\toprule
		 & \multicolumn{2}{c}{\textit{$\mathcal{R}_{H}$ Matter}} & \multicolumn{2}{c}{\textit{$\mathcal{R}_{H}$ Galaxy}}\\
 		\hline
		%\midrule
	 	      $z$               &  $NGC$ & $SGC$ & $NGC$ & $SGC$ \\
		\hline 

		$0.430-0.484$ & $64.2 \pm 1.3  $ & $66.7 \pm 1.6 $	& $126.4 \pm 11.4  $ & $121.1 \pm 9.8 $	\\
		$0.484-0.538$ & $65.4 \pm 0.9  $ & $63.9 \pm 1.5 $	& $111.9 \pm 4.9  $ & $119.8 \pm 8.8 $	\\
		$0.538-0.592$ & $62.6 \pm 0.8  $ & $65.2 \pm 1.6 $	& $116.4 \pm 7.8  $ & $110.5 \pm 5.1 $	\\
		$0.592-0.646$ & $60.4 \pm 0.8  $ & $60.1 \pm 1.1 $	& $108.8 \pm 3.9  $ & $120.1 \pm 11.7 $	\\
		$0.646-0.700$ & $59.0 \pm 0.8  $ & $60.1 \pm 1.8 $  & $125.8 \pm 7.3  $ & $147.4 \pm 8.4 $ \\
	 	\hline
		%\bottomrule
		\end{tabular}
		\end{center}
	\caption{\label{tab:RH-z} Homogeneity scale measurement $R^{\mathcal{D}_2=2.97}_{H}(z)$ as discribed by equation \ref{eq:RH-definition} for the galaxy and matter distributions for North and South galactic cap, fitted in scales $40 h^{-1}Mpc < r < 100 h^{-1}Mpc$.}
	\end{table}
	}

	%\paragraph{} We fit a simpler model for the relation between $R_{H}$ and $z$, $R^{SM}_{H}(z;A,\alpha)\ =\ A\ (1+z)^{-\alpha}$ resulting to $\alpha=0.63$ with a $\chi^{2}_{red} = 5.52/3$ for NGC and $\alpha=0.47$ with a $\chi^{2}_{red} = 2.9/3$ for SGC,suggesting that:
	%\begin{equation}
	%	R_{H} \propto \frac{1}{\sqrt{1+z}} = \sqrt{a}
	%\end{equation}
	%where $a$ is the scale factor.
	\vspace{10mm}
	
\end{comment}

%--------------------------------------------------------------------------------------------------------------------------------------------------
	\subsection{Consistency with $\Lambda$CDM} 
	
	In order to characterise more precisely the accordance with $\Lambda CDM$ model, we perform a fit to $1000$ mock catalogues and to data at scales $r\in[40,1300]h^{-1}Mpc$. The model we use is described by the following equation:
	\begin{equation}\label{eq:modelA}
		m(r;\alpha) = \mathcal{D}_2(\alpha r;\textbf{p}_{cosmo},\textbf{p}_{rsd})
	\end{equation}
	
	\begin{figure}[h!]
	\centering
	\includegraphics[width=100mm]{images/LCDM_d2_a_model.pdf}
	\caption{\label{fig:chi2-theory} Accordance of $\Lambda CDM$ model with the scale dependent \textit{fractal correlation dimension} $\mathcal{D}_2(r)$  using equation \ref{eq:modelA} at different redshift bins. The shaded areas correspond to the $1\sigma$ region computed from $1000$ QPM mock galaxy catalogues. See text for details}
	\end{figure}
	
	Using the fixed $\textbf{p}_{cosmo}$ and the measured $\textbf{p}_{rsd}$ parameters, we fit the $\alpha$-parameter. Deviations of $\alpha$-parameter will indicate excursions from $\Lambda CDM$ with \textbf{$p_{rsd}$}. The result of the fits are shown for different redshift bins for both NGC and SGC in figure \ref{fig:chi2-theory}. 
	

	{\color{blue}\paragraph{} The $\alpha$ values, all consistent with $1$, show the good agreement with $\Lambda CDM$ model, as it is demonstrated in figure \ref{fig:chi2-theory}. The colored shaded areas show the $1\sigma$ region away of the mean of $1000$ QPM mock catalogues. Furthermore, the $\chi^2$ obtained from those fits with $\Lambda CDM$ prediction are consistent with the number degrees of freedom 23 for the QPM mock catalogues. The grey shaded are on the bottom of figure \ref{fig:chi2-theory} indicates the $1\sigma$ region away from the expected $\chi_{exp}^2=23$. {\color{red}The mock catalogues follow exactly this pattern while we have a slight overestimation on the error on the parameter $\alpha$ on the largest redshift bin.} }
	
		
	%\vspace{100pt}
	\subsection{Constrains on Fractal Correlation Dimension}\label{subsect:ConD2}
	\paragraph{}	{\color{blue} In order to show the homogeneity of the CMASS DR12 sample on large scales we perform the following test. 

	In the range $300 h^{-1}Mpc < r < 1300 h^{-1}Mpc$, we take the average $\langle \mathcal{D}_2 \rangle-3$ accounting for the covariance matrix. in figure \ref{fig:D2zero}, we show that  $\langle \mathcal{D}_2 \rangle-3$ does not evolve with redshift. Then we take the effective mean over the $5$ redshift bins to constrain the Fractal correlation Dimension.}

	\begin{figure}[h!]
	\centering
	\includegraphics[width=100mm]{images/D2_Zero.png}
	\caption{\label{fig:D2zero} Fractal correlation dimension $\langle \mathcal{D}_2 \rangle-3$ averaged over $300 h^{-1}Mpc < r < 1300 h^{-1}Mpc$ for different redshift bins in the region $0.43\leq z \leq 0.7$ for the matter distribution.}	
	\end{figure}
	
	%{\color{blue} We find that for the \textit{str}-estimator for the galaxy distribution to be $3-\langle\mathcal{D}^{NGC}_{2}\rangle_{r,z} = (1.9 \pm 2.3) \times 10^{-3} $ and $3-\langle\mathcal{D}^{SGC}_{2}\rangle_{r,z} = (2.5 \pm 3.6)\times 10^{-3} $ at ($1\sigma$). While for the Matter distribution we have tighter constrains i.e. $3-\langle\mathcal{D}^{NGC}_{2}\rangle_{r,z} = (8.6 \pm 5.1)\times 10^{-4} $ and $3-\langle\mathcal{D}^{SGC}_{2}\rangle_{r,z} = (8.1 \pm 9.4) \times 10^{-4} $ at ($1\sigma$) .}

%	\begin{table}[h!]
%		\begin{center} 
%		\begin{tabular}{*5c} 
%		\hline
%		%\toprule
%		estim & \multicolumn{2}{c}{\textit{str}} & \multicolumn{2}{c}{\textit{cor}}\\
% 		\hline
%		%\midrule
%	 	$XGC$                      & $NGC$ & $SGC$ & $NGC$ & $SGC$ \\
%		\hline 
%		$Galaxy$                   & $6.4\times10^{-3}$ & $9.6\times10^{-3}$ & $2.5\times10^{-3}$ & $1.6\times10^{-4}$ \\
%		$Matter $                   & $1.9\times10^{-3}$ & $2.7\times10^{-3}$ & $3.2\times10^{-4}$ & $9.7\times10^{-5}$ \\
%	 	\hline
%		%\bottomrule
%		\end{tabular}
%		\end{center}
%	\caption{\label{tab:UpperLims} $2\sigma$-Upper limits for $3 - \langle\mathcal{D}_{2}\rangle_{r,z}$ for North and South galactic cap, for scales $250 h^{-1}Mpc < r < 1300 h^{-1}Mpc$.}
%	\end{table}

%	\begin{table}[h!]
%		\begin{center} 
%		\begin{tabular}{*5c} 
%		\hline
%		%\toprule
%		estim & \multicolumn{2}{c}{\textit{str}} & \multicolumn{2}{c}{\textit{cor}}\\
% 		\hline
%		%\midrule
%	 	$XGC$                      & $NGC$ & $SGC$ & $NGC$ & $SGC$ \\
%		\hline 
%		$Galaxy$                   & $(1.9\pm2.3)\times10^{-3}$ & $(2.5\pm3.6)\times10^{-3}$ & $(1.3\pm0.6)\times10^{-3}$ & $(4.1\pm5.7)\times10^{-4}$ \\
%		$Matter $                   & $(8.6\pm5.1)\times10^{-4}$ & $(8.1\pm9.4)\times10^{-4}$ & $(1.3\pm1.0)\times10^{-5}$ & $(0.1\pm4.8)\times10^{-5}$ \\
%	 	\hline
%		%\bottomrule
%		\end{tabular}
%		\end{center}
%	\caption{\label{tab:MeanD2} $2\sigma$-Upper limits for $3 - \langle\mathcal{D}_{2}\rangle_{r,z}$ for North and South galactic cap, for scales $250 h^{-1}Mpc < r < 1300 h^{-1}Mpc$.}
%	\end{table}

%	{\color{blue} We find tighter constrains for the \textit{cor}-estimator. For the galaxy distribution $3-\langle\mathcal{D}^{NGC}_{2}\rangle_{r,z} = (1.3 \pm 0.6)\times 10^{-3} $ and $3-\langle\mathcal{D}^{SGC}_{2}\rangle_{r,z} = (4.1 \pm 5.7)\times 10^{-4} $ at ($1\sigma$). While for the Matter distribution we have tighter constrains where $3-\langle\mathcal{D}^{NGC}_{2}\rangle_{r,z} = (1.3 \pm 1.0)\times 10^{-5} $ and $3-\langle\mathcal{D}^{SGC}_{2}\rangle_{r,z} = (0.1 \pm 4.8) \times 10^{-5} $ at ($1\sigma$) . The results are illustrated in table \ref{tab:MeanD2}}

	
%	{\color{blue} Finally, in table \ref{tab:UpperLims} , the $2\sigma$ upper limits are shown for the North and South Galactic Cap for the 2 different estimators and for the Galaxy and Matter distribution. We can observe that the \textit{cor}-estimator gives better constrains for the \textit{fractal correlation dimension} for both North and South galactic caps and for both galaxy and matter distribution. }

	{\color{blue} For the galaxy distribution $3-\langle\mathcal{D}^{NGC}_{2}\rangle_{r,z} = (1.1 \pm 5.4)\times 10^{-4} $ and $3-\langle\mathcal{D}^{SGC}_{2}\rangle_{r,z} = (0.7 \pm 1.1)\times 10^{-3} $ while for both $3-\langle\mathcal{D}^{NGC+SGC}_{2}\rangle_{r,z} = (9.0 \pm 4.8)\times 10^{-4} $ at ($1\sigma$). While for the Matter distribution we have tighter constrains where $3-\langle\mathcal{D}^{NGC}_{2}\rangle_{r,z} = (2.2 \pm 1.1)\times 10^{-4} $ and $3-\langle\mathcal{D}^{SGC}_{2}\rangle_{r,z} = (1.5 \pm 2.0)\times 10^{-4} $  and for both we have $3-\langle\mathcal{D}^{NGC+SGC}_{2}\rangle_{r,z} = (1.8 \pm 1.0)\times 10^{-4} $ at ($1\sigma$). The results are illustrated in table \ref{tab:MeanD2} for different redshift bins.}

{\small
	\begin{table}[h!]
		\begin{center} 
		\begin{tabular}{*5c} 
		\hline
%		estim & \multicolumn{2}{c}{\textit{str}} & \multicolumn{2}{c}{\textit{cor}}\\
% 		\hline
%		\toprule
		Distribution & \multicolumn{2}{c}{\textit{Matter}} & \multicolumn{2}{c}{\textit{Galaxy}}\\
 		\hline
		%\midrule
	 	      $z$               &  $NGC\ (\times 10^{-4})$ & $SGC\ (\times 10^{-4})$ & $NGC\ (\times 10^{-3})$ & $SGC\ (\times 10^{-3})$ \\
		\hline 

		$0.430-0.484$ & $-2.8 \pm 3.3  $ & $-2.5 \pm 8.1 $	& $-1.3 \pm 1.5  $ & $-1.1 \pm 3.7 $	\\
		$0.484-0.538$ & $-2.0 \pm 3.1  $ & $-1.9 \pm 5.4 $	& $-0.9 \pm 1.4  $ & $-0.8 \pm 2.4 $	\\
		$0.538-0.592$ & $-3.6 \pm 1.7  $ & $-2.4 \pm 9.9 $	& $-0.2 \pm 0.9  $ & $-1.2 \pm 4.9 $	\\
		$0.592-0.646$ & $-4.1 \pm 2.0  $ & $-0.9 \pm 4.5 $	& $-2.1 \pm 1.1  $ & $-0.5 \pm 2.3 $	\\
		$0.646-0.700$ & $-1.7 \pm 3.8  $ & $+0.2 \pm 2.8 $  & $-1.0 \pm 2.3  $ & $-0.1 \pm 1.6 $ \\
	 	\hline
		%\bottomrule
		\end{tabular}
		\end{center}
	\caption{\label{tab:MeanD2} Mean value with $1\sigma$ errors for $\langle\mathcal{D}_{2}\rangle_{r}(z)-3$ for North and South galactic cap, for scales $300 h^{-1}Mpc < r < 1300 h^{-1}Mpc$.}
	\end{table}
	}

	{\color{blue} The constrains on the matter distributions are slightly better than those of the galaxy distribution. This is in accordance with the fact that the total matter distribution is more clustered than the galaxy distribution which is just a tracer of the total matter of the universe.}	
	
	{\color{red} Making only the assumptions that were demonstrated in section \ref{subsec:RH-gal}, we can set a limit on the order of $\langle \mathcal{D}_2 \rangle - 3 =  7.12 \pm 3.75 \times 10^{-4}$ for matter distribution using only the Galaxy Distribution measurement of $\mathcal{D}_2$ which is compatible with what we measure in table \ref{tab:MeanD2}. } % NGC/sqrt(1.6)

